On Quantum Generalizations of Information-Theoretic Measures and their Contribution to Distributional Semantics

Information-theoretic measures such as relative entropy and correlation are extremely useful when modeling or analyzing the interaction of probabilistic systems. We survey the quantum generalization of 5 such measures and point out some of their commonalities and interpretations. In particular we find the application of information theory to distributional semantics useful. By modeling the distributional meaning of words as density operators rather than vectors, more of their semantic structure may be exploited. Furthermore, properties of and interactions between words such as ambiguity, similarity and entailment can be simulated more richly and intuitively when using methods from quantum information theory.

==> modeling.tex <==
\section{Modeling}

\subsection{Distributional Semantics}

\subsection{Formal Semantics}

\subsection{How Meaning Emerges from Modeling Choices}

\subsection{From Vectors to Density Matrices}

\subsection{Encoding Ambiguity}

==> references.tex <==
@string{ACL =    "Annual Meeting of the Association for Computational Linguistics"}
@string{COLING = "International Conference on Computational Linguistics"}
@string{EMNLP =    "Conference on Empirical Methods in Natural Language Processing"}
@string{ACLCOLING = "joint " # ACL # " and " # COLING  }


@Article{Schuetze:98,
  author =       {Hinrich Sch\"{u}tze},
  title =        {Automatic Word Sense Discrimination},
  journal =      {Computational Linguistics},
  year =         1998,
  volume =       24,
  number =       1,
  pages =        {97--124}
}

@InProceedings{choi01:latent,
  author =       {Freddy Choi and Peter Wiemer-Hastings and Johanna Moore},
  title =        {Latent {S}emantic {A}nalysis for text segmentation},
crossref = {EMNLP:01},
  pages =        {109-117}
}

@InProceedings{Lin:98,                                                          
  author =       {Dekang Lin},
  title =        {Automatic Retrieval and Clustering of Similar Words},
  crossref =     {COLING:ACL:98},
  pages =        {768--774},
  year =         1998}


@InProceedings{landaueretal1997,
  author = {Thomas K. Landauer and Darrell Laham and Bob Rehder and M. E. Schreiner},
  title = {How Well Can Passage Meaning be Derived without Using Word Order: A Comparison of Latent Semantic Analysis and Humans},
  booktitle = {{Proceedings of the 19th Annual Conference of the Cognitive Science Society}},
  year = {1997},
  pages = {412--417},
  publisher = {Lawrence Erlbaum Associates},
  address = {Mahwah NJ}
}

@phdthesis{mcdonald2000,
	author={Scott McDonald},
	year={2000},
	title={Environmental Determinants of Lexical Processing Effort.},
	school={University of Edinburgh}
}
@Article{Griffiths:Steyvers:07,
  author = 	 {Thomas L. Griffiths and Mark Steyvers and Joshua B. Tenenbaum},
  title = 	 {Topics in Semantic Representation},
  journal = 	 {Psychological Review},
  year = 	 2007,
  volume =	 114,
  number =	 2,
  pages =	 {211--244}
}

@article{foltzetal1998,
	author={Peter W. Foltz and Walter Kintsch and Thomas Landauer},
	title={The Measurement of Textual Coherence with Latent Semantic Analysis.},
	journal={Discourse Process},
	volume={15},
	pages={285--307},
	year={1998}
}
@PhdThesis{Laham:00,
  author = 	 {Darrell R. Laham},
  title = 	 {Automated Content Assessment of Text Using Latent Semantic Analysis to Simulate Human Cognition},
  school = 	 {University of Colorado at Boulder},
  year = 	 2000
}
@Proceedings{EMNLP:01,
  title =        {Proceedings of the 6th EMNLP},
  booktitle =    {Proceedings of the 6th EMNLP},
  year =         2001,
  address =      {Seattle, WA}
}
@InProceedings{COLING:ACL:98,                                                     
title = {Proceedings of the } # ACLCOLING,                                      
booktitle = {Proceedings of the } # ACLCOLING,                                  
  year = 1998,                                                                  
  address = {Montr\'{e}al, Canada}                                              
}     

@inproceedings{denhierelemaire2004,
	author={Denhi\`{e}re, Guy and Lemaire, Beno\^{i}t},
	year={2004},
	title={A Computational Model of Children's Semantic Memory},
	booktitle={{Proceedings of the 26th Annual Meeting of the Cognitive Science Society}},
	location={Chicago},
	publisher={Lawrence Erlbaum Associates},
	address={Mahwah, NJ},
	pages={297--302}
}
@article{lundburgess1996,
	author={Kevin Lund and Curt Burgess},
	year={1996},
	title={Producing high-dimensional semantic spaces from lexical co-occurrence.},
	journal={Behavior Research Methods, Instruments {\&} Computers},
	volume={28},
	pages={203--208}
 }

@Book{grefenstette94:explorations,
  author =       {Gregory Grefenstette},
  title =        {Explorations in Automatic Thesaurus Discovery},
  publisher =    {Kluwer Academic Publishers},
  year =         1994
}
@Article{Salton:ea:75,
  author = {G Salton and A Wang and C Yang},
  title = {A Vector-space Model for Information Retrieval},
  journal = {Journal of the American Society for Information Science},
  year = 1975,
  volume = 18,
  pages = {613--620}
}

@incollection{firth1957,
	author={John R. Firth},
	title={A synopsis of linguistic theory 1930-1955.},
	year=1957,
	booktitle={Studies in Linguistic Analysis},
	pages={1--32},
	publisher={Philological Society},
	address={Oxford}
}

@incollection{Socher:ea:2011,
 title ={Dynamic Pooling and Unfolding Recursive Autoencoders for Paraphrase Detection},
 author={Richard Socher and Eric H. Huang and Jeffrey Pennin and Andrew Y. Ng and Christopher D. Manning},
 booktitle = {Advances in Neural Information Processing Systems 24},
 editor = {J. Shawe-Taylor and R.S. Zemel and P. Bartlett and F.C.N. Pereira and K.Q. Weinberger},
 pages = {801--809},
 year = {2011}
}



@article{Pothos:Busemeyer:12,
  author = {Emmanuel M. Pothos and Jerome R. Busemeyer},
  title = {Can Quantum Probability Provide a New Direction for Cognitive Modeling?},
  publisher = {Cambridge University Press},
  journal = {Behavioral and Brain Sciences},
  year = {2012}
}


@Book{Khrennikov:10,
  author = 	 {Andrei Y. Khrennikov},
  title = 	 {Ubiquitous Quantum Structure: From Psychology to Finance},
  publisher = 	 {Springer},
  year = 	 2010}

@Book{Busemeyer:Bruza:12,
  author = 	 {Jerome R. Busemeyer and Peter D. Bruza},
  title = 	 {Quantum Models of Cognition and Decision},
  publisher = 	 {Cambridge University Press},
  address =      {Cambridge},
  year = 	 2012}

@Book{Isham:89,
  author = 	 {Chris J. Isham},
  title = 	 {Lectures on Quantum Theory},
   publisher = 	 {Singapore: World Scientific},
  year = 	 1989}

@Book{Hughes:89,
  author = 	 {R. I. G. Hughes},
  title = 	 {The Structure and Interpretation of Quantum Mechnics},
  publisher = 	 {Harvard University Press},
  year = 	 1989,
  address = 	 {Cambridge, MA}}

@Book{Nielsen:Chuang:10,
  author = 	 {Nielsen, Michael A. and Chuang, Isaac L.},
  title = 	 {Quantum Computation and Information Theory},
  publisher = 	 {Cambridge University Press},
  year = 	 2010,
  address = 	 {Cambridge}}

@Book{Baaquie:04,
  author = 	 {Belal E. Baaquie},
  title = 	 {Quantum Finance: Path Integrals and Hamiltonians for Oprions and Interest Rates},
  publisher = 	 {Cambridge University Press},
  year = 	 2004,
  address = 	 {Cambridge}}

@article{Aerts:09,
  author    = {Diederik Aerts},
  title     = {Quantum Structure in Cognition},
  journal   = {Journal of Mathematical Psychology},
  volume    = {53},
  pages	    = {314--348},
  year      = {2009}
}

@inproceedings{Bruza:05,
  author = {Peter D. Bruza and Richard J. Cole},
  title = {Quantum Logic of Semantic Space: An Exploratory Investigation of Context Effects in Practical Reasoning},
  booktitle = {We Will Show Them: Essays in Honour of Dov Gabbay},
  volume = {1},
  pages = {339--361},
  editor = {S. Artemov and H. Barringer and S. A. d'Avila Garcez and L. C. Lamb and J. Woods},
  publisher = {London: College Publications},
  year = {2005}
}

@inproceedings{Bruza:08,
  author = {Peter D. Bruza and Kirsty Kitto and Douglas McEnvoy and Cathy McEnvoy},
  year = {2008},
  title = {Entangling words and meaning},
  booktitle = {Second Quantum Interaction Symposium},
  publisher = {Oxford University}
}
@Article{Tversky:Kahneman:83,
  author = 	 {Amos Tversky and Daniel Kahneman},
  title = 	 {Extensional versus Intuitive Reasoning: The Conjuctive Fallacy in Probability Judgment},
  journal = 	 {Psychological Review},
  year = 	 1983,
  volume = 	 4,
  number = 	 90,
  pages = 	 {293--315}}


@Article{Tversky:Shafir:92,
  author = 	 {Amos Tversky and Eldar Shafir},
  title = 	 {The Disjunction Effect in Choice under Uncertainty},
  journal = 	 {Psychological Science},
  year = 	 1992,
  volume =   3,
  number = 	 5,
  pages = 	 {305--309}}



@Article{Aerts:Gabora:05,
  author = 	 {Diederik Aerts and Liane Gabora},
  title = 	 {A State-context-property Model of Concepts and their Combinations II: A Hilbert Space Representation.},
  journal = 	 {Kybernetes},
  year = 	 2005,
  volume = 	 {1--2},
  number = 	 34,
  pages = 	 {192--221}}


@Article{Bruza:ea:09,
  author = 	 {Peter D. Bruza and Kirsty Kitto and Douglas Nelson and Cathy McEvoy},
  title = 	 {Is there something quantum-like in the human mental lexicon?},
  journal = 	 {Journal of Mathematical Psychology},
  year = 	 2009,
  number = 	 5,
  volume =       53,
  pages = 	 {362--377}}

@inproceedings{Chen01b,
    author = {Joseph C.H. Chen and Manfred Kudlek},
    title = {Duality of Syntax and Semantics -- From the view point of brain as a quantum computer},
    booktitle = {Recent Advances in Natural Language Processing},
    address = {Tzigov Chark, Bulgarien},
    year = {2001}
}

@inproceedings{Chen01a,
    author = {Joseph C.H. Chen},
    title = {A Quantum Mechanical Approach to Cognition and Representation},
    booktitle = {Toward a Science of Consciousness},
    address = {Skövde, Sweden},
    year = {2001}
}

@phdthesis{Chen:diss,
	location = {http://www.scientificcommons.org/20264450},
	title = {Quantum computation and natural language processing},
	author = {Chen, Joseph C. H.},
	year = {2002},
	keywords = {Nat\"{u}rliche Sprache, Sprachverarbeitung, Common sense reasoning, Quantentheorie, Data processing Computer science, Sprachverarbeitung, K\"{u}nstliche Intelligenz},
	publisher = {Staats- und Universit\"{a}tsbibliothek Hamburg},
	url = {http://www.sub.uni-hamburg.de/opus/volltexte/2002/769/},
	institution = {E-Dissertationen der Universit\"{a}t Hamburg [http://www.sub.uni-hamburg.de/opus/oai/oai2.php] (Germany)},
	school = {Universit\"{a}t Hamburg}
}

@Article{Aerts:Czachor:04,
  author = 	 {Diederik Aerts and Marek Czachor},
  title = 	 {Quantum Aspects of Semantic Analysis and Symbolic Artificial Intelligence},
  journal = 	 {Journal of PhysicsA: Mathematical and General},
  year = 	 2004,
  volume = 	 37,
  pages = 	 {123--132}}

@article{landauerdumais1997,
	author={Thomas K. Landauer and Susan T. Dumais},
	year={1997},
	title={A solution to {Plato's} problem: the Latent Semantic Analysis theory of acquisition, induction and representation of knowledge.},
	journal={Psychological Review},
	volume={104},
	number={2},
	pages={211--240}}

@article{Coecke:ea:10,
  author    = {Bob Coecke and
               Mehrnoosh Sadrzadeh and
               Stephen Clark},
  title     = {Mathematical Foundations for a Compositional Distributional
               Model of Meaning},
  journal   = {CoRR},
  volume    = {abs/1003.4394},
  year      = {2010},
  ee        = {http://arxiv.org/abs/1003.4394},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{Gref:ea:11,
 title = "Concrete Sentence Spaces for Compositional Distributional Models of Meaning",
  author = "Edward Grefenstette and Mehrnoosh Sadrzadeh and Stephen Clark and Bob Coecke and Stephen Pulman",
  year = "2011",
  journal = "Proceedings of the 9th International Conference on Computational Semantics",
  pages = "125--134",
  url = "http://www.aclweb.org/anthology/W/W11/W11-0114.pdf"
}

@InProceedings{demarneffe-manning:2008:PE,
  author    = {de Marneffe, Marie-Catherine  and  Manning, Christopher D.},
  title     = {The {S}tanford Typed Dependencies Representation},
  booktitle = {Coling 2008: Proceedings of the workshop on Cross-Framework and Cross-Domain Parser Evaluation},
  year      = {2008},
  address   = {Manchester, UK},
  pages     = {1--8}
}


@misc {nelson1998norms,
  author = {Nelson, Douglas L. and McEvoy, Cathy L. and Schreiber, Thomas A.},
  year = {1998},
  title = {{The University of South Florida Word Association, Rhyme, and Word Fragment Norms}},
  url = {http://www.usf.edu/FreeAssociation/}
}

@article {finkelstein2002sim353,
  author = {Finkelstein, Lev and Gabrilovich, Evgeniy and Matias, Yossi and Rivlin, Ehud and Solan, Zach and Wolfman, Gadi and Ruppin, Eytan}, 
  title = {{Placing Search in Context: The Concept Revisited}},
  journal = {ACM Transactions on Information Systems},
  volume = {20},
  number = {1},
  pages = {116--131}, 
  month = {January},
  year = {2002}
}


@inproceedings{collobert_weston,
 author = {Collobert, Ronan and Weston, Jason},
 title = {A unified architecture for natural language processing: deep neural networks with multita\
sk learning},
 booktitle = {Proceedings of the 25th International Conference on Machine Learning},
 year = {2008},
 isbn = {978-1-60558-205-4},
 location = {Helsinki, Finland},
 pages = {160--167},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/1390156.1390177},
 doi = {10.1145/1390156.1390177},
 acmid = {1390177},
 publisher = {ACM},
 address = {New York, NY},
}
@Article{Bengio:ea:08,
  author =       {Yoshua Bengio},
  title =        {Neural Net Language Models},
  journal =      {Scholarpedia},
  year =         {2001},
  volume =       {3},
  number =      {1},
  pages =        {3881}
}
@Article{Baroni:Lenci:2010,
  author =       {Marco Baroni and Alessandro Lenci},
  title =        {Distributional Memory: A General Framework for Corpus-Based Semantics },
  journal =      {Computational Linguistics},
  year =         2010,
  volume =       36,
  number =       4,
  pages =        {673--721}}

@InProceedings{mitchell-lapata:2008:ACLMain,
  author    = {Mitchell, Jeff  and  Lapata, Mirella},
  title     = {Vector-based Models of Semantic Composition},
  booktitle = {Proceedings of ACL-08: HLT},
  year      = {2008},
  address   = {Columbus, Ohio},
  pages     = {236--244},
}

@article{Mitchell:Lapata:2010,
   author = {Jeff Mitchell and Mirella Lapata},
   title = {Composition in Distributional Models of Semantics},
   journal = {Cognitive Science},
   year = {2010},
   volume = {38},
   number = {8},
   pages = {1388--1429}

}
@InProceedings{blacoe-lapata:2012:EMNLP-CoNLL,
  author    = {Blacoe, William  and  Lapata, Mirella},
  title     = {A Comparison of Vector-based Representations for Semantic Composition},
  booktitle = {Proceedings of the 2012 Joint Conference on Empirical Methods in Natural Language Processing and Computational Natural Language Learning},
  year      = {2012},
  address   = {Jeju Island, South Korea},
  pages     = {546--556},
  url       = {http://www.aclweb.org/anthology/D12-1050}
}

@article{dirac1939,
author = {Dirac, Paul A. M.},
title = {A new notation for quantum mechanics},
journal = {Mathematical Proceedings of the Cambridge Philosophical Society},
volume = {35},
issue = {03},
issn = {1469-8064},
year = {1939},
pages = {416--418},
numpages = {3},
doi = {10.1017/S0305004100021162},
URL = {http://dx.doi.org/10.1017/S0305004100021162},
eprint = {http://journals.cambridge.org/article_S0305004100021162},
}

@Book{Vedral:06,
  author = 	 {Vlatko Vedral},
  title = 	 {Introduction to Quantum Information Science},
  publisher = 	 {Oxford University Press},
  year = 	 2006,
  address = 	 {New York}}

@Article{Kleppner:Jackiw:00,
  author = 	 {Daniel Kleppner and Roman Jackiw},
  title = 	 {One Hundred Years of Quantum Physics},
  journal = 	 {Science},
  year = 	 2000,
  volume = 	 289,
  number = 	 5481,
  pages = 	 {893--898}}


@Article{Osherson:Smith:81,
  author = 	 {Daniel Osherson and Edward E. Smith},
  title = 	 {On the Adequacy of Prototype Theory as a Theory of Concepts},
  journal = 	 {Cognition},
  year = 	 1981,
  volume = 	 9,
  pages = 	 {35--38}}



@InProceedings{silberer-lapata:2012:EMNLP-CoNLL,
  author    = {Silberer, Carina  and  Lapata, Mirella},
  title     = {Grounded Models of Semantic Representation},
  booktitle = {Proceedings of the 2012 Joint Conference on Empirical Methods in Natural Language Processing and Computational Natural Language Learning},
  year      = 2012,
  address   = {Jeju Island, South Korea},
  pages     = {1423--1433}
}
@InProceedings{huang-EtAl:2012:ACL20122,
  author    = {Huang, Eric  and  Socher, Richard  and  Manning, Christopher  and  Ng, Andrew},
  title     = {Improving Word Representations via Global Context and Multiple Word Prototypes},
  booktitle = {Proceedings of the 50th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  year      = {2012},
  address   = {Jeju Island, South Korea},
  pages     = {873--882},
  url       = {http://www.aclweb.org/anthology/P12-1092}
}

@inproceedings{turian,
 author = {Turian, Joseph and Ratinov, Lev and Bengio, Yoshua},
 title = {Word representations: a simple and general method for semi-supervised learning},
 booktitle = {Proceedings of the 48th Annual Meeting of the Association for Computational Linguistics},
 year = {2010},
 address = {Uppsala, Sweden},
 pages = {384--394}
}

@article{Frege:1892,
   author = {Frege, Gottlob}, 
   title = {{\"{U}ber Sinn und Bedeutung}}, 
   journal = {Zeitschrift f\"{u}r Philosophie und philosophische Kritik}, 
   volume = {100}, 
   pages = {25--50}, 
   year = {1892}
}

@inproceedings{Annesi12,
  author    = {Paolo Annesi and
               Valerio Storch and
               Roberto Basili},
  title     = {Space Projections as Distributional Models for Semantic
               Composition},
  booktitle = {CICLing (1)},
  year      = {2012},
  pages     = {323-335},
  ee        = {http://dx.doi.org/10.1007/978-3-642-28604-9_27}
}

@InProceedings{erkpado08,
  author =  {Katrin Erk and Sebastian Pad\'o},
  title =    {A Structured Vector Space Model for Word Meaning in Context},
  booktitle = {Proceedings of the 2008 Conference on Empirical Methods in Natural Language Processing},
  year = 2008,
  pages     = {897--906},
  address = {Honolulu, HI}
}

@inproceedings{Lowe01,
  author = {Lowe, Will},
  booktitle = {Proceedings of the 23rd Annual Meeting of the Cognitive Science Society},
  pages = {576--581},
  title = {Towards a theory of semantic space},
  address = {Edinburgh, Scotland},
  year = 2001
}

@book{Jolliffe:1986,
  author = {Jolliffe, I.T.},
  publisher = {Springer Verlag},
  title = {Principal Component  Analysis},
  year = 1986
}

@INPROCEEDINGS{Phillips2000,
    author = {P. Jonathon Phillips and Hyeonjoon Moon and Syed A. Rizvi and Patrick J. Rauss},
    title = {The FERET evaluation methodology for face recognition algorithms},
    booktitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
    year = {2000},
    volume = {22},
    number = {10},
    pages = {1090--1104}
}

@inproceedings{vandecruys2013,
	author = {Van de Cruys, Tim and Poibeau, Thierry and Korhonen, Anna},
  booktitle = {Proceedings of the 2013 Conference of the North American Chapter of the Association for Computational Linguistics: HLT},
  pages = {1142--1151},
  title = {A Tensor-based Factorization Model of Semantic Compositionality.},
  year = 2013,
  address = {Atlanta, GA}
}


@inproceedings{Grefenstette2011,
  author    = {Edward Grefenstette and
               Mehrnoosh Sadrzadeh},
  title     = {Experimental Support for a Categorical Compositional Distributional
               Model of Meaning},
  booktitle = {Proceedings of the 2011 Conference on Empirical Methods in Natural Language Processing},
  year      = {2011},
  pages     = {1394--1404},
  address = {Edinburgh, Scotland}
}

@InProceedings{blacoe-kashefi-lapata:2013:NAACL-HLT,
  author    = {Blacoe, William  and  Kashefi, Elham  and  Lapata, Mirella},
  title     = {A Quantum-Theoretic Approach to Distributional Semantics},
  booktitle = {Proceedings of the 2013 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technology},
  year      = {2013},
  address   = {Atlanta, GA},
  pages     = {847--857},
  url       = {http://www.aclweb.org/anthology/N13-1105}
}

@inproceedings{Lu2008,
  author = {Lu, Haiping and Plataniotis, Konstantinos N. and Venetsanopoulos, Anastasios N.},
  booktitle = {Proceedings of the 25th International Conference on Machine Learning},
  editor = {Cohen, William W. and McCallum, Andrew and Roweis, Sam T.},
  pages = {616--623},
  title = {Uncorrelated multilinear principal component analysis through successive variance maximization.},
  year = 2008
}


@INPROCEEDINGS{Lu2006,
    author = {Haiping Lu and K. N. Plataniotis and A. N. Venetsanopoulos},
    title = {Multilinear principal component analysis of tensor objects for recognition},
    booktitle = {Proceedings of the International Conference on Pattern Recognition},
    year = {2006},
    pages = {776--779},
    address = {Hong Kong, China}
}

@ARTICLE{Sarkar05,
    author = {Sudeep Sarkar and P. Jonathon Phillips and Zongyi Liu and Isidro Robledo Vega and Patrick Grother and Kevin W. Bowyer},
    title = {The {human ID} gait challenge problem: Data sets, performance, and analysis},
    journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
    year = {2005},
    volume = {27},
    pages = {162--177}
}

@incollection{SocherChenManningNg2013,
title = {Reasoning With Neural Tensor Networks for Knowledge Base Completion},
author = {Socher, Richard and Chen, Danqi and Manning, Christopher D. and Ng, Andrew},
booktitle = {Advances in Neural Information Processing Systems 26},
editor = {C.J.C. Burges and L. Bottou and M. Welling and Z. Ghahramani and K.Q. Weinberger},
pages = {926--934},
year = {2013},
url = {http://media.nips.cc/nipsbooks/nipspapers/paper_files/nips26/504.pdf}
}

@inproceedings{cohen2013,
    author = "Shay B. Cohen and Giorgio Satta and Michael Collins",
    title = "Approximate {PCFG} Parsing Using Tensor Decomposition",
    booktitle = "Proceedings of the 2013 Conference of the North American Chapter of the Association for Computational Linguistics: HLT",
    year = "2013",
    address = "Atlanta, GA"
}

@InProceedings{qiu2013,
  author    = {Qiu, Xipeng  and  Tian, Le  and  Huang, Xuanjing},
  title     = {Latent Semantic Tensor Indexing for Community-based Question Answering},
  booktitle = {Proceedings of the 51st Annual Meeting of the Association for Computational Linguistics},
  year      = {2013},
  address   = {Sofia, Bulgaria},
  pages     = {434--439}
}

@article{LuSurvey2011,
    author      = "Haiping Lu and  Konstantinos N. Plataniotis and Anastasios N. Venetsanopoulos",
    title       = "A Survey of Multilinear Subspace Learning for Tensor Data",
    journal     = "Pattern Recognition",
    volume      = "44",
    number      = "7",
    year        = "2011",
    pages       = "1540--1551"
}

@ARTICLE{Kolda09tensordecompositions,
    author = {Tamara G. Kolda and Brett W. Bader},
    title = {Tensor Decompositions and Applications},
    journal = {SIAM Review},
    year = {2009},
    volume = {51},
    number = {3},
    pages = {455--500}
}

@INPROCEEDINGS{Gale92,
    author = {William A. Gale and Kenneth W. Church and David Yarowsky},
    title = {One sense per discourse},
    booktitle = {DARPA Speech and Natural Language Workshop},
    year = {1992}
}

@InProceedings{VandeCruys2011,
  author    = {Van de Cruys, Tim},
  title     = {Two Multivariate Generalizations of Pointwise Mutual Information},
  booktitle = {Proceedings of the Workshop on Distributional Semantics and Compositionality},
  year      = {2011},
  address   = {Portland, OR},
  pages     = {16--20},
  url       = {http://www.aclweb.org/anthology/W11-1303}
}

@ARTICLE{Schuetze98,
    author = {Hinrich Sch\"{u}tze},
    title = {Automatic Word Sense Discrimination},
    journal = {Journal of Computational Linguistics},
    year = {1998},
    volume = {24},
    pages = {97--123}
}

@inproceedings{SocherEtAl2012:MVRNN,
author = {Richard Socher and Brody Huval and Christopher D. Manning and Andrew Y. Ng},
title = {Semantic Compositionality Through Recursive Matrix-Vector Spaces},
booktitle = {Proceedings of the 2012 Conference on Empirical Methods in Natural Language Processing}, 
year = 2012,
pages = {1201--1211},
address = {Jeju Island, South Korea}
}

@InProceedings{zanzotto2010,
  author    = {Zanzotto, Fabio Massimo  and  Korkontzelos, Ioannis  and  Fallucchi, Francesca  and  Manandhar, Suresh},
  title     = {Estimating Linear Models for Compositional Distributional Semantics},
  booktitle = {Proceedings of the 23rd International Conference on Computational Linguistics},
  year      = {2010},
  address   = {Beijing, China},
  pages     = {1263--1271}
}


@Article{Turney:Pantel:2010,
  author = 	 {Peter D. Turney and Patrick Pantel},
  title = 	 {From Frequency to Meaning: Vector Space Models of Semantics},
  journal = 	 {Journal of Artificial Intelligence Research},
  year = 	 2010,
  volume = 	 37,
  pages = 	 {141--188}}

@InProceedings{mikolov-yih-zweig:2013:NAACL-HLT,
  author    = {Mikolov, Tomas  and  Yih, Wen-tau  and  Zweig, Geoffrey},
  title     = {Linguistic Regularities in Continuous Space Word Representations},
  booktitle = {Proceedings of the 2013 Conference of the North American Chapter of the Association for Computational Linguistics: HLT},
  year      = {2013},
  address   = {Atlanta, GA},
  pages     = {746--751}
}

@Article{Collobert:ea:2011,
  author = 	 {Ronan Collobert and Jason Weston and L\'{e}on Bottou and Michael Karlen and Koray Kavukcuoglu and Pavel Kuksa},
  title = 	 {Natural Language Processing (Almost) from Scratch},
  journal = 	 {Journal of Machine Learning Research},
  year = 	 2011,
  volume = 	 12,
  pages = 	 {2493--2537}}


@Book{Manning:ea:2008,
  author = 	 {Christopher D. Manning and Prabhakar Raghavan and Hinrich Sch\"{u}tze},
  title = 	 {Introduction to Information Retrieval},
  publisher = 	 {Cambridge University Press},
  year = 	 2008,
  address = 	 {New York, NY}}


@Article{Sebastiani:2002,
  author = 	 {Fabrizio Sebastiani},
  title = 	 {Machine Learning in Automated
Text Categorization},
  journal = 	 {ACM Computing Surveys},
  year = 	 2002,
  volume = 	 34,
  pages = 	 {1--47}}

@InProceedings{yih-EtAl:2013:ACL2013,
  author    = {Yih, Wen-tau  and  Chang, Ming-Wei  and  Meek, Chistopher and  Pastusiak, Andrzej},
  title     = {Question Answering Using Enhanced Lexical Semantic Models},
  booktitle = {Proceedings of the 51st Annual Meeting of the Association for Computational Linguistics},
  year      = {2013},
  address   = {Sofia, Bulgaria},
  pages     = {1744--1753}
}


@InProceedings{Jones:ea:2006,
  author = 	 {Rosie Jones and  Benjamin Rey and Omid Madani and Wiley
Greiner},
  title = 	 {Generating Query Substititions},
  booktitle = {Proceedings of the 15th International Conference on the World-Wide Web},
  pages = 	 {387--396},
  year = 	 2006,
  address = 	 {Edinburgh, Scotland}}



@InCollection{Harris:1970,
  author = 	 {Zellig Harris},
  title = 	 {Distributional Structure},
  booktitle = 	 {Papers in Structural and Transformational Linguistics},
  pages = 	 {775--794},
  publisher = {Dordrecht, Holland: D. Reidel Publishing Company},
  year = 	 1970}
  
@article{Harris:1954,
  added-at = {2010-08-05T14:23:58.000+0200},
  author = {Harris, Zellig},
  biburl = {http://www.bibsonomy.org/bibtex/252e7950c31610617170d71c320f2252e/tgunkel},
  interhash = {a23596808b6273076e1259dedca16330},
  intrahash = {52e7950c31610617170d71c320f2252e},
  journal = {Word},
  key = {Harris},
  keywords = {diplom distributional},
  number = 23,
  pages = {146--162},
  timestamp = {2010-08-05T14:23:58.000+0200},
  title = {Distributional structure},
  volume = 10,
  year = 1954
}


@InProceedings{Baroni:Zamparelli:2010,
  author = 	 {Marco Baroni and Roberto Zamparelli},
  title = 	 {Nouns Are Vectors, Adjectives Are Matrices: Representing
Adjective-noun Constructions in Semantic Space},
  booktitle = {Proceedings of the 2010 Conference on Empirical Methods in Natural Language Processing},
  pages = 	 {1183--1193},
  year = 	 2010,
  address = 	 {Boston, MA}}


@Article{Bullinaria:Levy:07,
  author = 	 {John A. Bullinaria  and Joseph P. Levy},
  title = 	 {Extracting Semantic Representations from Word Co-occurrence Statistics: A Computational Study},
  journal = 	 {Behavior Research Methods},
  year = 	 2007,
  volume = 	 39,
  pages = 	 { 510--526}}

@InProceedings{socher-EtAl:2013:EMNLP,
  author    = {Socher, Richard  and  Perelygin, Alex  and  Wu, Jean  and  Chuang, Jason  and  Manning, Christopher D.  and  Ng, Andrew  and  Potts, Christopher},
  title     = {Recursive Deep Models for Semantic Compositionality Over a Sentiment Treebank},
  booktitle = {Proceedings of the 2013 Conference on Empirical Methods in Natural Language Processing},
  year      = {2013},
  address   = {Seattle, WA},
  pages     = {1631--1642}
}

@InProceedings{Widdows:2008,
  author = 	 {Dominic Widdows},
  title = 	 {Semantic Vector Products: Some Initial Investigations},
  booktitle = {Proceedings of the Second AAAI Symposium on Quantum Interaction},
  year = 	 2008,
  address = 	 {Glasgow, Scotland}}

@InProceedings{rudolph-giesbrecht:2010:ACL,
  author    = {Rudolph, Sebastian  and  Giesbrecht, Eugenie},
  title     = {Compositional Matrix-Space Models of Language},
  booktitle = {Proceedings of the 48th Annual Meeting of the Association for Computational Linguistics},
  year      = {2010},
  address   = {Uppsala, Sweden},
  pages     = {907--916}
}

@InProceedings{ji-eisenstein:2013:EMNLP,
  author    = {Ji, Yangfeng  and  Eisenstein, Jacob},
  title     = {Discriminative Improvements to Distributional Sentence Similarity},
  booktitle = {Proceedings of the 2013 Conference on Empirical Methods in Natural Language Processing},
  year      = {2013},
  address   = {Seattle, WA},
  pages     = {891--896},
  url       = {http://www.aclweb.org/anthology/D13-1090}
}

@InProceedings{fernando-stevenson:2008,
	author = {Fernando, S. and Stevenson, M.},
	year = 2008,
	title = {A semantic similarity approach to paraphrase detection},
	booktitle = {11th Annual CLUK Research Colloquium},
	address = {Oxford, UK}
}
@Article{Baroni:ea:2009,
  author = 	 {Marco Baroni and Silvia Bernardini and Adriano Ferraresi and Eros Zanchetta},
  title = 	 {The WaCky Wide Web: A Collection of Very Large Linguistically Processed Web-Crawled Corpora},
  journal = 	 {Language Resources and Evaluation},
  year = 	 2009,
  volume = 	 43,
  number =	 3,
  pages = 	 {209--226}}

@inproceedings{Schmid:1994,
  address = {Manchester, UK},
  author = {Schmid, Helmut},
  booktitle = {Proceedings of the International Conference on New Methods in Language Processing},
  title = {Probabilistic Part-of-Speech Tagging Using Decision Trees},
  year = 1994
}

@Article{Nivre:ea:2007,
  author = 	 {Joakim Nivre and Johan Hall and Jens Nilsson and Atanas Chanev and G\"{u}lsen Eryigit and Sandra K\"{u}bler and Svetoslav Marinov and Erwin Marsi},
  title = 	 {Maltparser: A Language Independent System for Data-driven Dependency Parsing},
  journal = 	 {Natural Language Engineering},
  year = 	 2007,
  volume = 	 13,
  number = 	 2,
  pages = 	 {95--135}}

@inproceedings{dolan-quirk-brockett:2004:COLING,
  author    = {Dolan, Bill  and  Quirk, Chris  and  Brockett, Chris},
  title     = {Unsupervised Construction of Large Paraphrase Corpora: Exploiting Massively Parallel News Sources },
  booktitle = {Proceedings of the 17th International Conference on Computational Linguistics},
  year      = 2004,
  address   = {Geneva, Switzerland},
  pages     = {350--356}
}


@Article{Hall:ea:2009,
  author = 	 {Mark Hall and Eibe Frank and Geoffrey Holmes and Bernhard Pfahringer and Peter Reutemann and Ian H. Witten},
  title = 	 {The WEKA Data Mining Software: An Update},
  journal = 	 {ACM SIGKDD Explorations Newsletter},
  year = 	 2009,
  volume = 	 11,
  number = 	 1,
  pages = 	 {10--18}}

@InProceedings{zeichner-berant-dagan:2012:ACL2012short,
  author    = {Zeichner, Naomi  and  Berant, Jonathan  and  Dagan, Ido},
  title     = {Crowdsourcing Inference-Rule Evaluation},
  booktitle = {Proceedings of the 50th Annual Meeting of the Association for Computational Linguistics},
  year      = {2012},
  address   = {Jeju Island, South Korea},
  pages     = {156--160}
}

@Article{Kotlerman:2010,
  author = 	 {Lili Kotlerman and Ido Dagan and Idan Szpektor and Maayan Zhitomirsky-Geffet},
  title = 	 {Directional Distributional Similarity for Lexical Inference},
  journal = 	 {Special Issue of Natural Language Engineering on Distributional Lexical Semantics},
  year = 	 2010,
  volume = 	 16,
  number = 	 4,
  pages = 	 {359--389}}

@InProceedings{melamud-EtAl:2013:Short,
  author    = {Melamud, Oren  and  Dagan, Ido  and  Goldberger, Jacob  and  Szpektor, Idan},
  title     = {Using Lexical Expansion to Learn Inference Rules from Sparse Data},
  booktitle = {Proceedings of the 51st Annual Meeting of the Association for Computational Linguistics},
  year      = {2013},
  address   = {Sofia, Bulgaria},
  pages     = {283--288}
}

@InProceedings{Diab:STS:2012,
  author = {Agirre, Eneko and Cer, Daniel and Diabm Mona and Gonzalez-Agirre, Aitor},
  title = {{SemEval-2012 Task 6: A} Pilot on Semantic Textual Similarity},
  year = {2012},
  booktitle = {Proceedings of the 1st Joint Conference on Lexical and Computational Semantics - Volume 1: Proceedings of the main conference and the shared task, and Volume 2: Proceedings of the Sixth International Workshop on Semantic Evaluation},
  address = {Montreal, Canada},
  pages = {385--393}
}

@InProceedings{Marelli:ea:2014,
  author = {Marco Marelli and Stefano Menini and Marco Baroni and Luisa Bentivogli and Raffaella Bernardi and Roberto Zamparelli},
  title = {A SICK Cure for the Evaluation of Compositional Distributional Semantic Models},
  booktitle = {Proceedings of the 9th International Conference on Language Resources and Evaluation},
  year = {2014},
  address = {Reykjavik, Iceland}
}


	

@InProceedings{Abend:ea:2014,
  author = 	 {Omri Abend and Shay B. Cohen and Mark Steedman},
  title = 	 {Lexical Inference over Multi-Word Predicates: A Distributional Approach},
  booktitle = {Proceedings of the  52nd Annual Meeting of the Association for Computational Linguistics},
  year = 	 2014,
  address = 	 {Baltimore, Maryland},
   pages     = {644--654},
}



@inproceedings{Weeds-Weir:2003:EMNLP,
  author = {Weeds, Julie  and  Weir, David},
  title  = {A General Framework for Distributional Similarity},
  booktitle = {Proceedings of the 2003 Conference on Empirical Methods in Natural Language Processing},
  year   = 2003,
  pages  = {81--88}, 
  address = {Sapporo, Japan}
}



@Article{Blei:ea:03,
  author = {Blei, D. M. and Ng, A. Y. and Jordan, M. I.},
  title = {Latent {Dirichlet} Allocation},
  journal = {Journal of Machine Learning Research},
  year = {2003},
  month = {January},
  volume = {3},
  pages = {993--1022}
}

@InProceedings{baroni-dinu-kruszewski:2014:P14-1,
  author    = {Baroni, Marco  and  Dinu, Georgiana  and  Kruszewski, Germ\'{a}n},
  title     = {Don't count, predict! A systematic comparison of context-counting vs. context-predicting semantic vectors},
  booktitle = {Proceedings of the 52nd Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  month     = {June},
  year      = {2014},
  address   = {Baltimore, Maryland},
  pages     = {238--247}
}

@InProceedings{pennington-socher-manning:2014:EMNLP2014,
  author    = {Pennington, Jeffrey  and  Socher, Richard  and  Manning, Christopher},
  title     = {Glove: Global Vectors for Word Representation},
  booktitle = {Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing},
  month     = {October},
  year      = {2014},
  address   = {Doha, Qatar},
  pages     = {1532--1543}}

@incollection{NIPS2013_5021,
title = {Distributed Representations of Words and Phrases and their Compositionality},
author = {Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg S and Dean, Jeff},
booktitle = {Advances in Neural Information Processing Systems 26},
editor = {C.J.C. Burges and L. Bottou and M. Welling and Z. Ghahramani and K.Q. Weinberger},
pages = {3111--3119},
year = {2013},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5021-distributed-representations-of-words-and-phrases-and-their-compositionality.pdf}
}

@Manual{sigf06,
  title = 	 {User's guide to \texttt{sigf}: Significance testing by 
                  approximate randomisation},
  author =	 {Sebastian Pad\'o},
  year =	 2006
}

@InProceedings{lai-hockenmaier:2014:SemEval,
  author    = {Lai, Alice  and  Hockenmaier, Julia},
  title     = {Illinois-LH: A Denotational and Distributional Approach to Semantics},
  booktitle = {Proceedings of the 8th International Workshop on Semantic Evaluation},
  year      = {2014},
  address   = {Dublin, Ireland},
  pages     = {329--334},
  url       = {http://www.aclweb.org/anthology/S14-2055}
}

@InProceedings{zhao-zhu-lan:2014:SemEval,
  author    = {Zhao, Jiang  and  Zhu, Tiantian  and  Lan, Man},
  title     = {ECNU: One Stone Two Birds: Ensemble of Heterogenous Measures for Semantic Relatedness and Textual Entailment},
  booktitle = {Proceedings of the 8th International Workshop on Semantic Evaluation (SemEval 2014)},
  year      = {2014},
  address   = {Dublin, Ireland},
  pages     = {271--277},
  url       = {http://www.aclweb.org/anthology/S14-2044}
}

@InProceedings{bjerva-EtAl:2014:SemEval,
  author    = {Bjerva, Johannes  and  Bos, Johan  and  van der Goot, Rob  and  Nissim, Malvina},
  title     = {The Meaning Factory: Formal Semantics for Recognizing Textual Entailment and Determining Semantic Similarity},
  booktitle = {Proceedings of the 8th International Workshop on Semantic Evaluation (SemEval 2014)},
  year      = {2014},
  address   = {Dublin, Ireland},
  pages     = {642--646}
}

@Book{Noreen:1989,
  author = 	 {Eric W. Noreen},
  title = 	 {Computer-intensive methods for testing hypotheses: an introduction},
  publisher = 	 {John Wiley and Sons, Inc},
  year = 	 1989}


@Article{Cohen:60,
  author = 	 {J Cohen},
  title = 	 {A Coefficient of Agreement for Nominal Scales },
  journal = 	 {Educational and Psychological Measurement},
  year = 	 1960,
  volume =	 20,
  pages =	 {37--46}
}

@article{Dimitri:Springer,
  title = "Compositional Operators in Distributional Semantics",
  author = "Dimitri Kartsaklis",
  year = "2014",
  issn = "2213-7793",
  journal = "Springer Science Reviews",
  doi = "10.1007/s40362-014-0017-z",
}

@unpublished{Robin2015,
	title = {Open System Categorical Quantum Semantics in Natural Language Processing},
	author = {Robin Piedeleu and Dimitri Kartsaklis and Bob Coecke and Mehrnoosh Sadrzadeh},
	year = {2015},
	note = {arXiv:1502.00831}
}

@unpublished{Esma2014,
	title = {Using Density Matrices in a Compositional Distributional Model of Meaning},
	author = {Esma Balkir},
	year = {2014},
	note = {Master's Thesis, University of Oxford}
}

@incollection{Sordoni2014,
year={2014},
isbn={978-3-642-54942-7},
booktitle={Quantum Interaction},
volume={8369},
series={Lecture Notes in Computer Science},
editor={Atmanspacher, Harald and Haven, Emmanuel and Kitto, Kirsty and Raine, Derek},
doi={10.1007/978-3-642-54943-4_13},
title={Looking at Vector Space and Language Models for IR Using Density Matrices},
url={http://dx.doi.org/10.1007/978-3-642-54943-4_13},
publisher={Springer Berlin Heidelberg},
author={Sordoni, Alessandro and Nie, Jian-Yun},
pages={147--159},
language={English}
}


@article{Coecke2010,
	year = {2010},
	title = {Mathematical Foundations for a Compositional Distributional Model of Meaning. Lambek Festschrift},
	author = {Bob Coecke and Mehrnoosh Sadrzadeh and Stephen Clark},
	journal = {Linguistic Analysis},
	volume = {36},
	pages = {345--384}
}

@incollection{Blacoe:QI2014,
year={2015},
isbn={978-3-319-15930-0},
booktitle={Quantum Interaction},
series={Lecture Notes in Computer Science},
editor={Atmanspacher, Harald and Bergomi, Claudia and Filk, Thomas and Kitto, Kirsty},
doi={10.1007/978-3-319-15931-7_4},
title={Semantic Composition Inspired by Quantum Measurement},
url={http://dx.doi.org/10.1007/978-3-319-15931-7_4},
publisher={Springer International Publishing},
author={Blacoe, William},
pages={41--53},
language={English}
}

@article{Werner1989,
  title = {Quantum states with Einstein-Podolsky-Rosen correlations admitting a hidden-variable model},
  author = {Werner, Reinhard F.},
  journal = {Phys. Rev. A},
  volume = {40},
  issue = {8},
  pages = {4277--4281},
  numpages = {0},
  year = {1989},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.40.4277},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.40.4277}
}

@unpublished{Vedral:RelativeEntropy,
	title = {The Role of Relative Entropy in Quantum Information Theory},
	author = {Vedral, Vlatko},
	year = {2001},
	note = {arXiv:quant-ph/0102094}
}

@unpublished{Vedral:Correlation,
	title = {Classical, quantum and total correlations},
	author = {Henderson, L and Vedral, V},
	year = {2001},
	note = {arXiv:quant-ph/0105028}
}

@article{Jensen:Inequality,
year={1906},
issn={0001-5962},
journal={Acta Mathematica},
volume={30},
number={1},
doi={10.1007/BF02418571},
title={Sur les fonctions convexes et les in\'egalit\'es entre les valeurs moyennes},
url={http://dx.doi.org/10.1007/BF02418571},
publisher={Kluwer Academic Publishers},
author={Jensen, J.},
pages={175-193},
language={French}
}

@Book{vonNeumann:1932,
  author =       "John von Neumann",
  title =        "{{Mathematische Grundlagen der Quantenmechanik}}",
  publisher =    "Springer",
  address =      "Berlin",
  year =         "1932",
  language =     "German",
}

@article {Erk:Survey:2012,
author = {Erk, Katrin},
title = {Vector Space Models of Word Meaning and Phrase Meaning: A Survey},
journal = {Language and Linguistics Compass},
volume = {6},
number = {10},
publisher = {Blackwell Publishing Ltd},
issn = {1749-818X},
url = {http://dx.doi.org/10.1002/lnco.362},
doi = {10.1002/lnco.362},
pages = {635--653},
year = {2012},
}

@article{Neumann1927,
author = {Neumann, J. von},
journal = {{Nachrichten von der Gesellschaft der Wissenschaften zu G\"ottingen, Mathematisch-Physikalische Klasse}},
language = {ger},
pages = {245--272},
title = {{Wahrscheinlichkeitstheoretischer Aufbau der Quantenmechanik}},
url = {http://eudml.org/doc/59230},
volume = {1927},
year = {1927},
}

@article{Vedral:discord,
  title = {The classical-quantum boundary for correlations: Discord and related measures},
  author = {Modi, Kavan and Brodutch, Aharon and Cable, Hugo and Paterek, Tomasz and Vedral, Vlatko},
  journal = {Rev. Mod. Phys.},
  volume = {84},
  issue = {4},
  pages = {1655--1707},
  numpages = {0},
  year = {2012},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.84.1655},
  url = {http://link.aps.org/doi/10.1103/RevModPhys.84.1655}
}

